Achieving Ultra-Reliable Low-Latency Communication (URLLC) in Next-Generation Cellular Networks with Programmable Data Planes

Recent advancements in wireless technologies towards the next-generation cellular networks have brought a new era that made it possible to apply cellular technology on traditionally-wired networks with tighter requirements, such as industrial networks. The next-generation cellular technologies (e.g., 5G and Beyond) introduce the concept of ultra-reliable low-latency communications (URLLC). This thesis presents a Software-Defined Networking (SDN) architecture with programmable data planes for the next-generation cellular networks to achieve URLLC. Our design deploys programmable switches between the cellular core and Radio Access Networks (RAN) to monitor and modify data traffic at the line speed. We introduce the concept of \textit{intra-cellular optimization}, a relaxation in cellular networks to allow pre-authorized in-network devices to communicate without being required to signal the core network. We also present a control structure, Unified Control Plane (UCP), containing a novel Ethernet Layer control protocol and an adapted version of link-state routing information distribution among the programmable switches. Our implementation uses P4 with an 5G implementation (Open5Gs) and a UE/RAN simulator. We implement a Python simulator to evaluate the performance of our system on multi-switch topologies by simulating the switch behavior. Our evaluation indicates latency reduction up to 2x with \textit{intra-cellular optimization} compared to the conventional architecture. We show that our design has a ten-millisecond level of control latency, and achieves fine-grained network security and monitoring.

==> donotinclude.tex <==
\begin{figure}
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-0.cm}
\ttfamily
\small
\begin{tabular}{r L L l}
    requirement &\rightarrow && (property, DHS)
    \\ && |& (requirement \& requirement)
    \\ property & \rightarrow & & (property $|$ property)
    \\ && | & (property \& property)
    \\ && | & ($\neg$ property)
    \\ && | & list(hop)
    \\ hop & \rightarrow & & [$d = D$] (device specifier)
    \\ && | & . (any device)
    \\ && | & * (zero or more of previous hop)
    \\ && | & $\hat{ }$ (beginning of path)
    \\ && | & \$ (end of path)
    \\ && | & $<$ (local device)
    \\ && | & $>$ (packet destination)
    \\ DHS & \rightarrow && list(wildcard)
    \\ wildcard & \rightarrow & & $p \in \{0,1,^*\}^L$
\end{tabular}
\caption{}\label{fig:}
\end{figure}

\begin{figure}
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-0.cm}
\ttfamily
\small
\begin{tabular}{|c|c|c|}
    \hline
    & Name & Description \\ \hline
    1 & .srcMAC & Source MAC address. \\ \hline
    2 & .dstMAC & Destination MAC address. \\ \hline
    3 & .srcIP & Source IP (v4 or v6) address. \\ \hline
    4 & .dstIP & Destination IP (v4 or v6) address. \\ \hline
    5 & .srcPort & Source port number (TCP or UDP). \\ \hline
    6 & .dstPort & Destination port number (TCP or UDP). \\ \hline
    7 & .devices & A dictionary of devices with \\
    & &  their role (e.g., required, end of path) \\ \hline

\end{tabular}
\caption{Control Plane Framework library properties for a packet. Each property can take a single value, a range or an inequality.}\label{fig:cp}
%\reducespace
\end{figure}

==> fbe-reference.tex <==
\chapter{EXPERIMENTS AND RESULTS}
\label{chapter:experiments-and-results}

Experiments and results come here... 
\section{Sample Section}
Always place some text after headings before putting a graphics into a section as seen in Figure~\ref{fig:sinAndCosineSample}. 

\begin{figure}[htbp]
	\begin{center}
		\includegraphics[width=0.5\columnwidth]{sample_figure.png}
		\vskip\baselineskip % Leave a vertical skip below the figure
		\caption{Sin and Cosine.}
		\label{fig:sinAndCosineSample}
	\end{center}
\end{figure}

Also, below, you can find how to arrange figures that can span multiple pages.

Descriptive text explaining Figure~\ref{fig:sampleWithContinuation}. Notice that even though Figure~\ref{fig:sampleWithContinuation} is on the following page, descriptive text can reside in a former page as long as the figure number is referenced. \\ \\ \\ \\ \\


Descriptive text explaining the continuation of Figure~\ref{fig:sampleWithContinuation}. Normally FBE expects this page to be fully filled with content, hence the need for shifting text from following pages into here.

Now, let us cite some studies: one source as \cite{doebelin},  two
sources as \cite{doebelin,exoplanetwebsite} or you may cite three or
more sources as 
\cite{doebelin,exoplanetwebsite,aran2007databaseofnon-manual}.\nocite{
	liudissertation} \nocite{paper-IAT-2006-labels}
Observe that they are ordered in the references chapter in the same
order as
they are cited. Both the IEEE referencing and APA referencing methods are allowed, this document uses IEEE reference style, for more info on APA, check~\cite{libraryguideswebsite}. Also, note that since the URL is long, LaTeX has trouble in manually linebreaking, hence a modification is made in the references.bib file.

\begin{figure}[h]
	\begin{center}
		\includegraphics[width=\textwidth, keepaspectratio]{sample_figure_with_continuation.pdf}
		\caption{Sample Figure}
		\label{fig:sampleWithContinuation}
		\vskip\baselineskip
	\end{center}
\end{figure}

\clearpage
\begin{center}
	\includegraphics[width=\textwidth, keepaspectratio]{sample_figure_with_continuation_2.pdf}
		Figure 2.2. Sample Figure (cont.)
	\vskip\baselineskip
\end{center}

 Let us put a sample table as seen in Table~\ref{table:shortTable}. Please pay attention that the caption is followed
by a period.

\begin{table}[thbp]
%\vskip\baselineskip 
\caption[Sample table]{Sample table.}
\begin{center}
\begin{tabular}{|c|c|c|} \hline
 & \textbf{Header 1}& \textbf{Header 2}\\\hline
\textbf{Row 1} & Bla bla bla& Bla bla bla \\\hline
\textbf{Row 2} & Bla bla bla  & Bla bla bla \\\hline
\end{tabular}
\label{table:shortTable}
\end{center}
\end{table}

Next up, there is a sample table that spans multiple pages. Normally the packages that are used for this breaks the formatting package provided by FBE, but if done like this, you won't encounter the ``package conflict" error stated in the FrequentlySeenMistakes.pdf in the FBE web site.
\clearpage

\begin{table}[thbp]
	\caption[Sample table that spans multiple pages.]{Sample table that spans multiple pages.}
	\label{table:multiPageSample}
\end{table}
\begin{center}
	\addtocounter{table}{-1}
	\begin{longtable}{|l|l|}\hline
		\endfirsthead
		\multicolumn{2}{c}{Table \ref{table:multiPageSample}. Sample table that spans multiple pages. (cont.) \vspace{1em}} \\\hline
		\endhead
		\endfoot
		\endlastfoot
		
		\textbf{Header 1}& \textbf{Header 2}\\\hline
		Bla bla bla & Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\\hline
		
		Bla bla bla & Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\\hline
		
		Bla bla bla & Bla bla bla \\
		& Bla bla bla \\\hline
		Bla bla bla & Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\\hline
		
		\pagebreak
		\textbf{Header 1}& \textbf{Header 2}\\\hline
		Bla bla bla & Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\\hline
		
		Bla bla bla & Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\\hline
		
		Bla bla bla & Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\
		& Bla bla bla \\\hline
	\end{longtable}
\end{center}
\vskip -2cm %This is used to remove excessive space after the longtable. It's not mandatory, can be removed if the final output isn't as desired.

You can use the code of Table~\ref{table:multiPageSample} to create multiple page spanning longtables.

Footnotes should be avoided as possible. If there is an absolute
necessity, footnotes should be used as this.\footnote{Example of a
footnote}  Please be informed that URLs are not allowed within thesis text, even in footnotes. Provide them as citations instead.

\clearpage
Item lists may be represented as follows:

\begin{itemize}
 \item This is an item. Do not use boldface for the items.
\begin{enumerate}
 \item This is a sub-item. Subsub-items are not allowed.
\end{enumerate}
\item Another item.
\end{itemize}
%  \item 
% \end{enumerate}

Item lists may also be represented as follows:
\begin{enumerate}
 \item This is another enumerated item.
\begin{itemize}
 \item This is another sub-item.
\end{itemize}

\end{enumerate}

\begin{thm}
The solutions of the equation $ax^2+bx+c=0$ with $a\neq 0$ are
$$
x=\frac{-b\pm \sqrt{b^2-4ac}}{2a}
$$
\end{thm}


\begin{proof}
We use the method of completing the square to rewrite $ax^2+bx+c$.
\begin{align*}
ax^2+bx+c&=a\left( x^2 + \frac{b}{a}x+\right)+c \\
  &=a\left( x^2 + \frac{b}{a}x+ \left(\frac{b}{2a}\right)^2
     -\left(\frac{b}{2a}\right)^2 +\right)+c \\
  &=a\left( x+\frac{b}{2a}\right)^2 - 
a\left(\frac{b}{2a}\right)^2+c\\
  &= a\left( x+\frac{b}{2a}\right)^2- \frac{b^2-4ac}{4a}
\end{align*}
Therefore $ax^2+bx+c=0$ can be rewritten as 
$$
a\left( x+\frac{b}{2a}\right)^2- \frac{b^2-4ac}{4a}=0
$$
which can in turn  be rearranged as
$$
\left( x+\frac{b}{2a}\right)^2= \frac{b^2-4ac}{4a^2}
$$
Taking square roots gives
$$
x+\frac{b}{2a}= \frac{\pm \sqrt{b^2-4ac}}{2a}
$$
which implies
$$
x=\frac{-b\pm \sqrt{b^2-4ac}}{2a}
$$
as required.
\end{proof}
Finally, we will put a sample algorithm (PCA algorithm) using the
relevant package in a figure as shown in Figure \ref{alg:pca} and
sample equations.

\begin{figure}[htbp]
\label{alg:pca}
\begin{center}
\framebox[6.0in]{\begin{minipage}[t]{5.9in}
\begin{algorithmic}
\STATE
\STATE \textbf{Require}  $\mathbf{s_i},\ i=1,2,\dots,N$ are normalized
 
\STATE Compute the mean  $\mathbf{\bar{s}}$ using Eq. \ref{eq:mean};
\STATE Form the $N\times2L$ matrix $\mathbf{Q}$ as defined in Eq.
\ref{eq:q};
\IF{ $N < 2\times L$}
\STATE $\mathbf{Q} \Leftarrow \mathbf{Q}^T$ ;
\ENDIF
\STATE Compute the covariance matrix $\mathbf{C}_s$ using Eq.
\ref{eq:cov_matrix};\STATE Decompose $\mathbf{C}_s$
 to its eigenvectors   $\mathbf{e}_k$  and eigenvalues $\lambda_k$
satisfying Eq. \ref{eq:pca};
\IF{ $N < 2\times L$}
\FOR{$k=1$ to $K$}
\STATE $\mathbf{e}_k \Leftarrow \mathbf{Q}\mathbf{e}_k $ ;
\STATE $\mathbf{e}_k \Leftarrow \mathbf{e}_k/||\mathbf{e}_k|| $
(normalization);
\ENDFOR
\ENDIF
\STATE
\end{algorithmic}
\end{minipage}}
\end{center}
\caption[Principal Component Analysis Algorithm]{Principal Component
Analysis Algorithm.}
% \vskip
\end{figure}

\begin{align} 
\mathbf{\bar{s}} & =\frac{1}{N} \sum_{i=1}^N \mathbf{s}_i
\label{eq:mean}   
\\
\mathbf{Q} & =\left[ 
\begin{array}{cccc} 
 \mathbf{s}_1  - \mathbf{\bar{s}} & \mathbf{s}_2 - \mathbf{\bar{s}} &
\cdots & \mathbf{s}_N  - \mathbf{\bar{s}}
\end{array}
\right]_{2L\times N }
\label{eq:q}
\\ 
\mathbf{C}_s & =\frac{1}{N} \mathbf{Q}^T \mathbf{Q}
\label{eq:cov_matrix}
\end{align}

\begin{equation}
    \mathbf{C}_s \mathbf{e}_k = \lambda_k \mathbf{e}_k
    \label{eq:pca}
\end{equation}

\subsection{Example of First Subheadings}
Some text here
\subsubsection{Example of Second Subheadings}
Some text here too.
\chapter{CONCLUSION}
\label{chapter:conclusion}

The conclusions of the thesis should come
here.
% \nocite{NewEntry1,NewEntry2,NewEntry3,NewEntry4,NewEntry5,
% NewEntry6,
% NewEntry7,NewEntry8,NewEntry9,NewEntry10,NewEntry11,NewEntry12}
